Sapiens: Foundation for Human Vision Models

We present Sapiens, a family of models for four fundamental human-centric vision tasks -- 2D pose estimation, body-part segmentation, depth estimation, and surface normal prediction. Our models natively support 1K high-resolution inference and are extremely easy to adapt for individual tasks by simply fine-tuning models pretrained on over 300 million in-the-wild human images. We observe that, given the same computational budget, self-supervised pretraining on a curated dataset of human images significantly boosts the performance for a diverse set of human-centric tasks. The resulting models exhibit remarkable generalization to in-the-wild data, even when labeled data is scarce or entirely synthetic. Our simple model design also brings scalability -- model performance across tasks improves as we scale the number of parameters from 0.3 to 2 billion. Sapiens consistently surpasses existing baselines across various human-centric benchmarks. We achieve significant improvements over the prior state-of-the-art on Humans-5K (pose) by 7.6 mAP, Humans-2K (part-seg) by 17.1 mIoU, Hi4D (depth) by 22.4% relative RMSE, and THuman2 (normal) by 53.5% relative angular error. Project page: https://about.meta.com/realitylabs/codecavatars/sapiens.

==> tables/7_data_size.tex <==
\begin{table}[ht]
\centering
\captionsetup{font=small}
\vspace{-0.2in}
\resizebox{3.8in}{!}{
    \setlength{\tabcolsep}{6pt}
    \renewcommand{\arraystretch}{1.1}
    
    \begin{tabular}{l|c|cccc}
    \toprule
    \textbf{Pretraining Data Source} & \textbf{\#Images} & \textbf{Pose} ($\uparrow$) &  \textbf{Seg}($\uparrow$) &  \textbf{Depth}($\downarrow$)  & \textbf{Normal}($\downarrow$)  \\
\midrule
Random & - & 20.1 & 9.6 & 0.720 & 35.4\\
ImageNet1K~\cite{russakovsky2015imagenet} & 1.2M & 42.5 & 18.4 & 0.466 & 27.0\\
COCO (non-human)\cite{lin2014microsoft} & 273K & 40.2 & 20.3 & 0.419 & 28.1\\
COCO (human)\cite{lin2014microsoft} & 150K & 50.8 & 28.7 & 0.304 & 25.5\\
COCO + AIC (human)~\cite{wu2017ai} & 500K & 52.6 & 29.6 & 0.330 & 26.3\\
Humans-300M (Ours) & 300M & \textbf{63.5} & \textbf{34.8} & \textbf{0.288} & \textbf{21.8}\\
    \bottomrule
    \end{tabular}
}


\vspace{0.05in}
\caption{Comparison of Sapiens-0.3B pretrained on various data sources. A domain-specific pretraining yields superior results compared to general data sources.}
\vspace{-0.3in}
\label{table:data_size}
\end{table}

